Provably Stable Flux Reconstruction High-Order Methods on Curvilinear Elements

Provably stable flux reconstruction (FR) schemes are derived for partial differential equations cast in curvilinear coordinates. Specifically, energy stable flux reconstruction (ESFR) schemes are considered as they allow for design flexibility as well as stability proofs for the linear advection problem on affine elements. Additionally, split forms are examined as they enable the development of energy stability proofs. The first critical step proves, that in curvilinear coordinates, the discontinuous Galerkin (DG) conservative and non-conservative forms are inherently different--even under exact integration and analytically exact metric terms. This analysis demonstrates that the split form is essential to developing provably stable DG schemes on curvilinear coordinates and motivates the construction of metric dependent ESFR correction functions in each element. Furthermore, the provably stable FR schemes differ from schemes in the literature that only apply the ESFR correction functions to surface terms or on the conservative form, and instead incorporate the ESFR correction functions on the full split form of the equations. It is demonstrated that the scheme is divergent when the correction functions are only used for surface reconstruction in curvilinear coordinates. We numerically verify the stability claims for our proposed FR split forms and compare them to ESFR schemes in the literature. Lastly, the newly proposed provably stable FR schemes are shown to obtain optimal orders of convergence. The scheme loses the orders of accuracy at the equivalent correction parameter value c as that of the one-dimensional ESFR scheme.

==> body/Abstract_Intro_Conclusion/abstract.tex <==

PLEASE REFER TO MAIN.TEX FOR SOME REASON IT WON"T LET ME INPUT THE ABSTRACT, SO I MANUALLY WROTE IT THERE!

Provably stable flux reconstruction (FR) schemes are derived for partial differential equations cast in curvilinear coordinates for, uncollocated, modal, split forms with different volume and surface cubature nodes. Specifically, energy stable flux reconstruction (ESFR) schemes are considered as they allow for design flexibility as well as stability proofs for the linear advection problem on affine elements. %As the ESFR stability proofs have solely been shown on affine meshes, they are limited therein. 
Additionally, split forms have recently seen a resurgence in research activity due to their resultant nonlinear (entropy) stability proofs. The first critical step proves that the discontinuous Galerkin (DG) curvilinear conservative and non-conservative forms are inherently different, even under exact integration and analytically exact metric terms; deeming the split form essential for curvilinear high-order schemes. Subsequently, this leads to the construction of metric dependent ESFR correction functions in each element. Furthermore, the provably stable FR schemes differ from the literature as the incorporate the ESFR correction functions on the volume integrals, and it is proven that no stability claim can be made using only a surface reconstruction. We numerically verify the stability claims for our proposed FR split forms in contrast to ESFR schemes in the literature. Lastly, the new proposed provably stable FR schemes are shown to obtain the correct orders of accuracy, and have the orders of accuracy drop off at the exact same location as the one-dimensional ESFR schemes.


\iffalse
Moreover, FR schemes, specifically energy stable FR (ESFR) schemes also known as Vincent-Castonguay-Jameson-Huynh schemes, have proven attractive as they allow for design flexibility as well as stability proofs for the linear advection problem on affine elements. Additionally, split forms have recently seen a resurgence in research activity due to their resultant nonlinear (entropy) stability proofs. This paper derives for the first time nonlinearly stable ESFR schemes in split form that enable nonlinear stability proofs for, uncollocated, modal, ESFR split forms with different volume and surface cubature nodes. The critical enabling technology is applying the splitting to the discrete stiffness operator. This naturally leads to appropriate surface and numerical fluxes, enabling both entropy stability and conservation proofs. When these schemes are recast in strong form, they differ from schemes found in the ESFR literature as the ESFR correction functions are incorporated on the volume integral. Furthermore, numerical experiments are conducted verifying that the new class of proposed ESFR split forms is nonlinearly stable in contrast to the standard split form ESFR approach. Lastly, the new ESFR split form is shown to obtain the correct orders of accuracy.

\fi

\iffalse

{From Previous version TO BE CHANGED}In this paper, provably linearly stable (energy stable) flux reconstruction (FR) schemes are built for partial differential equations cast 
in curvilinear coordinates. The one parameter family of flux reconstruction (FR) schemes is shown to be equivalent to a dense-norm summation-by-parts discretization. This recast allows the use of a staggered approach to construct linearly 
stable schemes, where metrics and derivatives are computed on flux nodes and the solution is computed on solution nodes. 
Alternatively, a staggered metrics approach is developed where  derivatives are computed on the solution nodes while 
metrics are computed on the flux nodes. The staggered approach fits naturally within an finite element code base, while 
the staggered metric approach is more closely aligned with collocated discretizations; future work will examine the relative merits of these approaches and efficient implementations. The theoretical 
properties of the schemes are verified by simulating the two-dimensional convection equation using the Huynh FR scheme 
with Gauss solution nodes and Gauss Lobatto flux nodes of the same degree. 
\fi

==> body/ESFR_Section/ESFR_Vol_Corr.tex <==
\subsection{ESFR with Volume Correction Functions}

Alike~\cite{zwanenburg_equivalence_2016}, we first introduce the facet correction field,

\begin{equation}
    h^{f,k}(\bm{\xi}^r) =\frac{1}{J_m^\Omega} \nabla^r\cdot \bm{g}^{f,k}(\bm{\xi}^r).
\end{equation}

\noindent where we included the determinant of the Jacobian since it is technically a contravariant correction field.
After projecting to the polynomial basis and evaluating at volume cubature nodes, we can represent the correction field exactly with  polynomial basis of order $3p$ alike~\cite{zwanenburg_equivalence_2016},

\begin{equation}
    \bm{\chi}(\bm{\xi}_v^r) (\hat{\bm{h}}^{f,k})^T = \bm{J}_m^{-1}\nabla^r\cdot \bm{g}^{f,k}(\bm{\xi}_v^r).\label{eq: Corr field def}
\end{equation}

Next, we return to Eq.~\ref{eq: CURV ESFR fund assumpt} (the ESFR fundamental assumption on curvilinear grids) and integrate the first volume term by parts,

\begin{equation}
\int_{\bm{\Gamma}_r}\bm{\chi}(\bm{\xi}^r)^T \Big(\hat{\bm{n}}^r\cdot
     \bm{g}^{f,k}(\bm{\xi}^r)\Big) d\bm{\Gamma}_r
   - \int_{\bm{\Omega}_r} \bm{\chi}(\bm{\xi}^r)^T \nabla^r\cdot
     \bm{g}^{f,k}(\bm{\xi}^r) d\bm{\Omega}_r  
    - c\int_{\bm{\Omega}_r}\frac{\partial^{3p}\bm{\chi}(\bm{\xi}^r) ^T}{\partial \xi^p\partial \eta^p\partial \zeta^p} J_m^\Omega
   \frac{\partial^{3p}}{\partial \xi^p\partial \eta^p\partial \zeta^p}\Big( \frac{1}{J_m^\Omega}\nabla^r \cdot \bm{g}^{f,k}(\bm{\xi}^r)\Big)d\bm{\Omega}_r =\bm{0}^T.
\end{equation}

Recalling Eq.~\ref{eq: ESFR conditions} from definition, rewriting in operator form and bringing the second and third integrals to the right hand side,

\begin{equation}
    \bm{\chi}(\bm{\xi}_{f,k}^r)^T W_{f,k}
    = \bm{\chi}(\bm{\xi}_{v}^r)^T \bm{W} \bm{J}_m \bm{J}_m^{-1} 
    \nabla^r\cdot
     \bm{g}^{f,k}(\bm{\xi}_v^r)
     + c \frac{\partial^{3p}\bm{\chi}(\bm{\xi}_v^r) ^T}{\partial \xi^p\partial \eta^p\partial \zeta^p} \bm{J}_m\bm{W}
   \frac{\partial^{3p}}{\partial \xi^p\partial \eta^p\partial \zeta^p}\Big( \bm{J}_m^{-1}\nabla^r \cdot \bm{g}^{f,k}(\bm{\xi}_v^r)\Big).
\end{equation}

Substituting Eq.~\ref{eq: Corr field def},

\begin{equation}
  \Big(\bm{M}_m+\bm{K}_m\Big) \Big(\hat{\bm{h}}^{f,k}\Big)^T = \bm{\chi}(\bm{\xi}_{f,k}^r)^T W_{f,k}.\label{eq: facet corr equiv cond}
\end{equation}

Thus Eq.~\ref{eq: facet corr equiv cond} is an equivalent presentation of the ESFR fundamental assumption Eq.~\ref{eq: CURV ESFR fund assumpt}. We derived this form to now present the much needed definition of an ESFR volume correction field. Similarly to Eq.~\ref{eq: facet corr equiv cond}, we introduce the newly proposed ESFR fundamental assumption for a volume correction field $ \bm{\chi}(\bm{\xi}_v^r) (\hat{\bm{h}}^{v})^T = \bm{J}_m^{-1}\nabla^r\cdot \bm{g}^{v}(\bm{\xi}_v^r)$ as,

\begin{equation}
    \Big(\bm{M}_m+\bm{K}_m\Big) \Big(\hat{\bm{h}}^{v}\Big)^T = \bm{\chi}(\bm{\xi}_{v}^r)^T \bm{W}.\label{eq: vol corr equiv cond}
\end{equation}

That is, we have the volume correction field's condition recovers a volume integral in Eq.~\ref{eq: vol corr equiv cond} whereas the facet correction field's condition recovers a facet integral in Eq.~\ref{eq: facet corr equiv cond}.



Thus, using the proposed volume correction field, our proposed ESFR split form is,

\begin{equation}
    \begin{split}
       \bm{\chi}(\bm{\xi}_v^r) \frac{d}{dt}\hat{\bm{u}}_m(t)^T 
    +\frac{1}{2} \bm{\chi}(\bm{\xi}_v^r)\Big(\hat{\bm{h}}^v\Big)^T
    \nabla^r\cdot \bm{\chi}(\bm{\xi}_v^r)\hat{\bm{f}}_{m}^{r}(t)^T
    +\frac{1}{2} \bm{\chi}(\bm{\xi}_v^r)\Big(\hat{\bm{h}}^v\Big)^T
    \bm{C}_m\nabla^r\cdot \bm{\chi}(\bm{\xi}_v^r)\hat{\bm{f}}_{m}(t)^T\\
    +\bm{\chi}(\bm{\xi}_v^r)\Big(\hat{\bm{h}}^{f,k}\Big)^T[\hat{\bm{n}}^r\cdot \bm{f}_m^{C,r}]   =\bm{0}^T.
    \end{split}\label{eq: ESFR split corr field}
\end{equation}

Please recall that we included the inverse of the determinant within the contravariant correction fields. 

The energy prove works out perfectly by using Equations ~\ref{eq: facet corr equiv cond} and~\ref{eq: vol corr equiv cond}.

Next we prove that for a linear flux the volume correction field has no influence for all correction functions satisfying Eq.~\ref{eq: vol corr equiv cond}, but for a nonlinear flux it has an influence. Also, $\bm{\chi}(\bm{\xi}_v^r)\Big(\hat{\bm{h}}_{DG}^v\Big)^T=\bm{J}_m^{-1}$ in proof.

\textbf{proof not typed up at the moment but I've wirtten it up}

==> body/SBP/SBP_operators.tex <==
\section{Review of tensor-product SBP operators}\label{sec:SBP}

\textcolor{red}{I have no clue how to write up their face lifting properly}
Relating SBP operators to previous formulation, volume and facet cubature nodes are "flux nodes". The basis functions are considered as Lagrange polynomials. Thus, the interpolating operator is the basis function.

\textcolor{red}{previous paper copy pasted below}


SBP operators are matrix difference operators approximating derivatives at mesh nodes; they can be characterized 
in terms of their degree, which is the degree of monomial for which they are exact. In this paper, the 
word order is reserved to refer to the order of convergence of the solution error and the accuracy of the discretization is exclusively 
discussed in terms of degree. The definition of a one-dimensional SBP operator in the $\xil$ direction is~\cite{DCDRF2014,Fernandez2014} 
\begin{definition}\label{SBP}
\textbf{Summation-by-parts operator for the first derivative}: A matrix operator,
$\DxiloneD\in\mathbb{R}^{N_{p}\times N_p}$, 
is an SBP operator approximating the derivative $\frac{\partial}{\partial \xil}$ on the nodal distribution $\xil\in\left[\alpha_{l},\beta_{l}\right]$, 
of degree p if 
\begin{enumerate}
\item $\DxiloneD\bm{\xi}_{l}^{k}=k\bm{\xi}_{l}^{k-1}$, $k=0,1,\dots,p$;
\item $\DxiloneD\equiv\left(\HxiloneD\right)^{-1}\QxiloneD$, where the norm matrix,$\HxiloneD$, is symmetric 
positive definite, and; 
\item $\QxiloneD\equiv\left(\SxiloneD+\frac{1}{2}\ExiloneD\right)$, where $\SxiloneD=-\left(\SxiloneD\right)\Tr$, $\ExiloneD=\left(\ExiloneD\right)\Tr$, and $\ExiloneD$ satisfies 

$\left(\bm{\xi}_{l}^{i}\right)\Tr\ExiloneD\bm{\xi}_{l}^{j} = \beta_{l}^{i+j}-\alpha_{l}^{i+j}$, $i,\,j=0,1,\dots,r$, $r\ge p$,
\end{enumerate}
with the convention that $\bm{\xi}_{l}^{k}=\bm{0}$ for $k<0$.
\end{definition}
For the purpose of imposing boundary conditions or inter-element coupling using SATs, it is convenient to decompose $\ExiloneD$ as 
\cite{DCDRF2014}
%
\begin{equation*}
\ExiloneD = \tbetal\tbetal\Tr-\talphal\talphal\Tr,
\end{equation*}
%
where 
%
\begin{equation*}
\talphal\Tr\bm{\xil}^{k}=\alpha_{l}^{k},\quad\tbetal\Tr\bm{\xil}^{k}=\beta_{l}^{k},\quad k=0,1,\dots,r.
\end{equation*}
%
The tensor-product extension to three dimensions of the one-dimensional SBP operators is given as 
%
\begin{equation*}
\Dxione \equiv \DxioneoneD\otimes\Ixitwo\otimes\Ixithree,\quad\Dxitwo \equiv \Ixione\otimes\DxitwooneD\otimes\Ixithree,
\quad \Dxitwo \equiv \Ixione\otimes\Ixitwo\otimes\DxithreeoneD,
\end{equation*}
%
where $\Ixil$ are identity matrices of size $\Nl\times\Nl$ for $l=1,\,2,\,3$.
For the purpose of analysis, it is convenient rewrite the tensor-product operators in the following way:

\begin{equation}\label{recast}
\begin{array}{lll}
\M\equiv\HxioneoneD\otimes\HxitwooneD\otimes\HxithreeoneD,&\\
\Dxione\equiv\M^{-1}\Qxione,&\Qxione\equiv\QxioneoneD\otimes\HxitwooneD\otimes\HxithreeoneD,&
%\Dxitwo\equiv\M^{-1}\Qxitwo,&\Qxitwo\equiv\HxioneoneD\otimes\QxitwooneD\otimes\HxithreeoneD,\\
%\Dxithree\equiv\M^{-1}\Qxithree,&\Qxithree\equiv\HxioneoneD\otimes\HxitwooneD\otimes\QxithreeoneD,\\\\
\Exione\equiv\Ebetaone+\Ealphaone,\\
\Ebetaone\equiv\Rbetaone\Tr\Mxioneperp\Rbetaone,&
\Ealphaone\equiv-\Ralphaone\Tr\Mxioneperp\Ralphaone,&\Mxioneperp\equiv\HxitwooneD\otimes\HxithreeoneD\\
%\Exitwo\equiv\Ebetatwo+\Ealphatwo,\\
%\Ebetatwo=\Rbetatwo\Tr\Mxitwoperp\Rbetatwo,&
%\Ealphatwo\equiv-\Ralphatwo\Tr\Mxitwoperp\Ralphatwo,&\Mxitwoperp\equiv\HxioneoneD\otimes\HxithreeoneD\\
%\Exithree\equiv\Ebetathree+\Ealphathree,\\
%\Ebetathree=\Rbetathree\Tr\Mxithreeperp\Rbetathree,&
%\Ealphathree\equiv-\Ralphathree\Tr\Mxithreeperp\Ralphathree,&\Mxithreeperp\equiv\HxioneoneD\otimes\HxitwooneD\\\\
\Rbetaone\equiv\tbetaone\Tr\otimes\Ixitwo\otimes\Ixithree,&
\Ralphaone\equiv\talphaone\Tr\otimes\Ixitwo\otimes\Ixithree,\\
%\Rbetatwo\equiv\Ixione\otimes\tbetatwo\Tr\otimes\Ixithree,&
%\Ralphatwo\equiv\Ixione\otimes\talphatwo\Tr\otimes\Ixithree,\\
%\Rbetathree\equiv\Ixione\otimes\Ixitwo\otimes\tbetathree\Tr,&
%\Ralphathree\equiv\Ixione\otimes\Ixitwo\otimes\talphathree\Tr.
\end{array}
\end{equation}
%
where the remaining directions are similarly recast. 

The discretization of the one-dimensional convection equation~\eqref{eq:1Dconvectioncurv} proceeds by 
approximating the derivative of the flux using the SBP operator and adding a weak imposition of 
boundary conditions or inter-element coupling using SATs giving 
\begin{equation}\label{eq:1DSBP}
\frac{\mr{d}\uk}{\mr{d}t}+a\DxioneD\uk+\M^{-1}\tL\left(a\tL\Tr\uk-\FLdI\right)
-\M^{-1}\tR\left(a\tR\Tr\uk-\FRdI\right)=0,
\end{equation}
where the term left multiplied by $\M^{-1}\tL$ is the SAT that couples the $\kappa$ element to the $\kappa-1$ element and 
the term left multiplied by $\M^{-1}\tR$ is the SAT that couples the $\kappa$ element to the $\kappa+1$ element. Furthermore, 
the resulting SBP-SAT scheme is equivalent to the FR scheme with $\gL=-\M^{-1}\tL$ and $\gR=\M^{-1}\tR$.



\subsection{The Staggered Approach}

\subsection{The Staggered Metric Approach}


\subsection{Equivalence of All the Above Approaches}

1) Equiv through projection
2) Equiv SBP with VAr DG from flux nodes as cubature nodes
3) Equiv ESFR with DG from $c_{DG}=0$

